Intra and Cross-spectrum Iris Presentation Attack Detection in the NIR and Visible Domains

Iris Presentation Attack Detection (PAD) is essential to secure iris recognition systems. Recent iris PAD solutions achieved good performance by leveraging deep learning techniques. However, most results were reported under intra-database scenarios and it is unclear if such solutions can generalize well across databases and capture spectra. These PAD methods run the risk of overfitting because of the binary label supervision during the network training, which serves global information learning but weakens the capture of local discriminative features. This chapter presents a novel attention-based deep pixel-wise binary supervision (A-PBS) method. A-PBS utilizes pixel-wise supervision to capture the fine-grained pixel/patch-level cues and attention mechanism to guide the network to automatically find regions where most contribute to an accurate PAD decision. Extensive experiments are performed on six NIR and one visible-light iris databases to show the effectiveness and robustness of proposed A-PBS methods. We additionally conduct extensive experiments under intra-/cross-database and intra-/cross-spectrum for detailed analysis. The results of our experiments indicates the generalizability of the A-PBS iris PAD approach.

==> Makefile <==
# Created by Sebastien Marcel <marcel@idiap.ch> 
# Wed 12 Apr 15:18:46 CEST 2017

# Builds the LaTeX project as a PDF document

TEXFILE=author.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex 
	latex $(@:%.pdf=%.tex)
	makeindex -s svind.ist author.idx
	makeindex -t author.glg -o author.gls -s myglo.ist author.glo
	@if [ -e references.bib ]; then \
	 bibtex $(@:%.pdf=%); \
	 latex $(@:%.pdf=%); \
	fi
	latex $(@:%.pdf=%.tex)
	dvipdf author

all: $(PDFFILE)

.PHONY: clean 

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.gls *.glg *.dvi *.ps *.pdf *.out *.brf

